Keypoint Promptable Re-Identification

Occluded Person Re-Identification (ReID) is a metric learning task that involves matching occluded individuals based on their appearance. While many studies have tackled occlusions caused by objects, multi-person occlusions remain less explored. In this work, we identify and address a critical challenge overlooked by previous occluded ReID methods: the Multi-Person Ambiguity (MPA) arising when multiple individuals are visible in the same bounding box, making it impossible to determine the intended ReID target among the candidates. Inspired by recent work on prompting in vision, we introduce Keypoint Promptable ReID (KPR), a novel formulation of the ReID problem that explicitly complements the input bounding box with a set of semantic keypoints indicating the intended target. Since promptable re-identification is an unexplored paradigm, existing ReID datasets lack the pixel-level annotations necessary for prompting. To bridge this gap and foster further research on this topic, we introduce Occluded-PoseTrack ReID, a novel ReID dataset with keypoints labels, that features strong inter-person occlusions. Furthermore, we release custom keypoint labels for four popular ReID benchmarks. Experiments on person retrieval, but also on pose tracking, demonstrate that our method systematically surpasses previous state-of-the-art approaches on various occluded scenarios. Our code, dataset and annotations are available at https://github.com/VlSomers/keypoint_promptable_reidentification.

==> figures/data_augmentation.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.6\linewidth]{figures/assets/data_augmentation.pdf}
  \caption{
    Our proposed Batch-wise Inter-Person Occlusion (BIPO) data augmentation creates artificial person occlusions that are consistent across image, prompt, and human parsing labels.
    BIPO is crucial to enforce the model to rely on the input prompts.
  }
\label{fig:data_augmentation}
\end{figure}


==> figures/dataset_figure.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.6\linewidth]{figures/assets/posetrack_reid.pdf}
  \caption{
    (a) Three identities from our proposed {\OccPT} dataset.
    (b) and (c) illustrates our proposed keypoints annotations for two popular occluded and holistic ReID datasets.
  }
\label{fig:dataset_figure}
\end{figure}


==> figures/rebuttal_figure.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\linewidth]{figures/assets/rebuttal_figure.pdf}
  \caption{
      Ranking when prompting the front/back person. 
      % Colored heatmaps illustrate the attention maps of KPR, with one color per part.
      % Only queries's prompt and attention maps are displayed here.
      Colored pastel dots are positive keypoints prompt with one color per body part ({\ra}), and small red dots are negative keypoints prompt.
      In real scenarios, it is the responsibility of the upstream human operator or pose model (e.g. for pose tracking) to indicate the target person.
  }
\label{fig:pull_figure}
\end{figure}


==> sections/7_acknowledgments.tex <==
\paragraph{Acknowledgment}
% \section*{ACKNOWLEDGMENT}
% UCLouvain + EPFL + Sport Radar | Synergy Sports
This work has been funded by Sportradar, by the Walloon region project ReconnAIssance, and by the Fonds de la RechercheScientifique – FNRS.

